IMBench: A Benchmark for Intuitive Robotic Manipulation

Humans combine reasoning and motor control to solve complex manipulation tasks under diverse constraints. They build an understanding of the physical world that helps them convert reasoning into actions and quickly adapt to new scenes, tasks, and rules. We refer to this capability as intuitive manipulation. Existing benchmarks fail to capture this integration: they evaluate physical reasoning in isolation from execution, or measure policy performance without requiring explicit reasoning. We introduce IMBENCH, a benchmark designed to evaluate intuitive manipulation as an integrated capability spanning perception, physical reasoning, action generation, and iterative execution. Our tasks require models to infer task-relevant physical structure and generate feasible action sequences under explicit constraints, including contact-rich manipulation, tool use, and multi-stage dependencies. We introduce a benchmark of 35 tasks, 14K filtered trajectories, and scalable tools for generating diverse scenarios. Experiments reveal a consistent gap: vision language models show partial physical reasoning ability but fail to produce executable plans, while state-of-the-art vision-language-action models struggle to satisfy task constraints and generalize across scenarios. These results identify intuitive manipulation as a missing axis in current foundation models and generalist robot policies, and position IMBENCH as a step toward evaluating and enabling more integrated, adaptive physical intelligence.

==> scratch.tex <==

% =====================================================================
\section{VLM Evaluation Details}
\label{sec:vlm_evaluation}
 
The vision language model (VLM) evaluation pipeline comprises two sequentially executed stages, each independently assessed. Stage~1 evaluates visual constraint extraction from multi-view scene frames and structured metadata, while Stage~2 assesses high-level plan generation conditioned on the output of Stage~1. Detailed prompt templates for both stages are provided in the supplementary materials.
 
\subsection{Implementation Details and Agent Design}
 
The IMBAgent operates through a two-stage architectural design that progressively grounds task planning in physical constraints derived from visual observation and sensor data.
 
In Stage~1, the agent receives multi-view camera frames of the scene alongside task descriptions, robot configuration parameters, and sensor signals (e.g., force and tactile feedback). The agent processes this information to extract physical constraints essential for task completion, such as robot mobility characteristics, motion restrictions imposed by the scene geometry, and robot-specific constraints relevant to the task. The output of Stage~1 is a constraint memory artifact---a structured representation grounding the plan in observed physical reality rather than generic procedural knowledge. This artifact maintains both episodic memory (frame-by-frame observations from each camera view) and semantic memory (facts extracted from observations, such as object contact relationships, functional roles, and critical physical properties). The artifact explicitly documents information that cannot be inferred from visual input alone, indicating what must be confirmed through sensor feedback during execution. This explicit separation of known and unknown information ensures that Stage~2 operates with full awareness of its knowledge boundaries.
 
In Stage~2, the agent receives the Stage~1 constraint artifact along with the original scene and sensor data. The agent treats all content in the Stage~1 artifact as inviolable constraints that must guide planning. Stage~2 operates through its own reasoning loop, using the extracted constraints and evidence as episodic memory and leveraging the physical facts as semantic memory to establish a grounded understanding of the scene. The agent then reasons about causal and temporal dependencies between actions, using the Stage~1 constraints to establish a partial order over required steps. This reasoning produces an ordered sequence of sub-goals, where each sub-goal specifies: (1)~the physical state to be achieved, (2)~preconditions that must hold before execution, (3)~postconditions expected after completion, and (4)~the specific Stage~1 constraint that necessitates this step. The complete sequence of sub-goals constitutes the procedural memory of the task---not merely a collection of facts about the scene, but the actionable knowledge required to execute the task step by step. All intermediate artifacts are preserved: prompts, frames, reasoning traces, validation logs, and explicit constraint links. As multiple task instances are executed, the episodic records accumulate into generalizable semantic knowledge that can be leveraged by future planning instances.
 
\subsection{Stage~1: Constraint Extraction via ReAct}
 
Stage~1 employs a Reason + Act (ReAct) based agent architecture. At each reasoning step, the agent first articulates why a particular constraint is relevant, then determines the specific constraints that must be satisfied when addressing it. Before reasoning commences, the agent loads all requisite information into its context window, establishing a working memory that persists across all reasoning iterations for a given task instance. This memory contains task instructions, timestamped camera frames, robot configuration, and sensor readings.
 
The reasoning process unfolds in four phases:
\begin{enumerate}
    \item \textbf{Observation:} The agent systematically examines each camera view, reviews sensor data, and ingests the task description.
    \item \textbf{Reasoning:} The agent asks itself structured questions: What objects are present in the scene? Where are they located? Are there task-specific constraints or tricks imposed by scene configuration?
    \item \textbf{Constraint Ranking:} Identified constraints are prioritized according to their impact on task success, with task-critical constraints ranked highest.
    \item \textbf{Verification:} Each constraint claim is validated against actual observed frames or metadata facts to prevent hallucinations or unsupported inferences.
\end{enumerate}
 
Should the quality check fail, the agent re-executes the stage, with each attempt logged for traceability. The final output is a well-defined constraint memory artifact documenting both episodic observations (what was seen frame-by-frame across cameras) and semantic facts (object relationships, roles, and physical properties).
 
\subsection{Stage~2: Constrained Plan Generation via ReAct}
 
Stage~2 receives the Stage~1 constraint artifact alongside the original scene and sensor data. The agent treats every element in this artifact as a rule that the plan must obey. Stage~1 constraints and evidence function as episodic memory, while physical facts function as semantic memory, providing grounded understanding of the scene for planning.
 
Stage~2 executes its own ReAct loop by loading constraints, hidden state flags, and infeasible actions into working memory. The agent reasons about action dependencies and causal ordering, using Stage~1 constraints to establish a valid partial order of steps. From this reasoning, the agent generates an ordered list of sub-goals, each specifying the physical achievement target, required preconditions, expected postconditions, and the originating Stage~1 constraint. This sequence of sub-goals constitutes the procedural memory---the step-by-step knowledge of how to execute the task. All artifacts are preserved: prompts, frames, reasoning chains, validation audits, and constraint links. As multiple task executions accumulate, episodic observations convert into reusable semantic knowledge for subsequent planning episodes.
 



\subsection{Stage~3: Closed-Loop Execution via VLM-Driven ReAct}
\label{app:stage3}

Stage~3 implements the live execution layer of the IMBAgent, realising the plan produced in Stage~2 through a closed-loop \textbf{ReAct (Reasoning + Acting)} cycle. At each decision step, the VLM is presented with the full current state of the robot and scene---expressed as structured text and camera images---and must select exactly one motor primitive to execute. The simulator advances by the number of ticks required for that primitive to converge, and the resulting state becomes the observation for the next step, creating a tight sense--decide--act loop that continues until the task succeeds, a budget is exhausted, or the VLM signals completion.

\subsubsection*{State Representation}

A central challenge in deploying VLMs for physical manipulation is converting high-dimensional robot state into a form legible to a language model. Stage~3 addresses this through a \textbf{structured textual observation summary} assembled at the start of every step. This summary is a configurable composition of sensor channels: end-effector pose (position in metres, quaternion, and roll/pitch/yaw in degrees), gripper openness percentage, a six-axis wrist force-torque reading in both sensor and world frames, per-object names and poses derived from the MuJoCo model, and camera calibration metadata. Each channel is individually togglable, allowing the information density of each prompt to be tuned to the task.

When object sensing is enabled, every physically present object in the scene is described on a single line with its world-frame position, orientation, and physical extents in metres (e.g.\ width~$\times$~depth~$\times$~height). Object dimensions are resolved at runtime from MuJoCo geometry, preferring labelled visual geoms over collision proxies. The summary header explicitly reports the count of \emph{visible} objects so the VLM is aware of the filtering.

\subsubsection*{Visual Grounding and Temporal Context}

Text alone cannot convey spatial relationships or gripper--object proximity. Stage~3 therefore supplements the observation summary with camera images from four viewpoints: an eye-in-hand gripper camera for close-range approach assessment, and three fixed exocentric cameras (front, right, left) providing global scene layout and depth disambiguation. All four images are captured at the start of every step and appended to the prompt as base64-encoded JPEGs.

A single snapshot provides no information about motion trajectory. To give the VLM temporal awareness, Stage~3 maintains a \textbf{rolling frame history} of the last $H$ camera batches (default $H{=}12$). The images supplied to the VLM at step $t$ are therefore the ordered sequence of batches from steps $t{-}H$ through $t$, oldest first. A dedicated \texttt{frames\_section} segment in the prompt labels each batch by step number and marks the final batch as current, ensuring the VLM acts on the latest state rather than a historical one. Each additional history batch adds approximately 1,800 input tokens; the rolling window causes the per-step token count to plateau at roughly 28,500 tokens after step $H$, bounding input cost independently of episode length.

\subsubsection*{Prompt Architecture}

Every VLM call is driven by a single \textbf{slot-based prompt template} populated at runtime with seven injectable sections: the current step number and budget, the task identifier, a natural-language goal and constraint description specific to the task, the structured observation summary, the frame-batch description, and the working memory of recent steps. The prompt is intentionally self-contained---every call carries the full task specification, the full current state, and the full relevant history, with no reliance on implicit cross-call session state.

A substantial portion of the template is devoted to \textbf{robot-specific reference documentation} that is static across all tasks. This covers the world-frame coordinate convention, the canonical table height ($z \approx 0.82$\,m), key end-effector height landmarks (home: 1.2\,m; safe transit: 1.05\,m; hover: 0.95--1.0\,m; grasp/place: 0.82--0.86\,m), gripper kinematics and openness encoding, controller action scaling, and a catalogue of common failure modes (sideways gripper, missed grasp, XY drift during vertical moves). This embedded documentation ensures the VLM has sufficient domain knowledge to plan physically plausible actions without fine-tuning or retrieval augmentation. It is re-supplied at every step because the VLM's context window is stateless from the system's perspective.

\subsubsection*{Action Space and Primitive Vocabulary}

The VLM does not produce raw joint commands. Instead, it selects from a small vocabulary of \textbf{named motion primitives}, each of which is a goal-directed action that abstracts away the underlying control loop. The vocabulary comprises eight primitives: \textsc{MoveEEF} (move the end-effector to a world-frame target position and optional orientation), \textsc{CloseGripper}, \textsc{OpenGripper}, \textsc{Lift} (raise by a vertical offset), \textsc{Descend} (lower to a target $z$-height holding $x,y$), \textsc{AtomicAction} (raw 7D action vector for $N$ simulator ticks), \textsc{Hold} (maintain current pose), and \textsc{Done} (signal task completion).

All primitive arguments use the world frame, matching the coordinate system reported in the observation summary. Frame conversion to the robot's base frame is handled transparently inside the control layer. The most frequently used primitive, \textsc{MoveEEF}, implements a proportional control loop that exits early once both positional error (threshold: 5\,mm) and orientation error (threshold: 5°) drop below tolerance, so the VLM specifies a \emph{step budget} rather than an exact duration.

The Primitives layer maintains a per-robot \textbf{gripper state register}: the most recently commanded open/close state is inherited by all movement primitives automatically, preventing the common failure mode where a grasped object is dropped mid-transport due to an implicit gripper reset.

\subsubsection*{VLM Integration via Native Tool Use}

Stage~3 is provider-agnostic, supporting OpenAI (Responses API), Anthropic (Messages API), Google Generative AI, and AWS Bedrock via a common request/response protocol. The preferred interaction mode is \textbf{native function calling}: the eight primitives are registered as typed JSON function schemas, and the VLM is instructed via \texttt{tool\_choice: required} to return exactly one tool call per step. This ensures provider-side schema validation rejects malformed calls before they reach the execution layer, and structurally separates action type, parameters, and reasoning in the response. Each tool schema mandates three top-level fields---\texttt{reasoning}, \texttt{description}, and \texttt{params}---so every action is accompanied by a language explanation that can be logged and inspected. When a provider does not support native tool use, the pipeline falls back to schema-constrained structured output and then to regex-backed free-form JSON parsing.

For OpenAI's Responses API, Stage~3 implements \textbf{stateful response threading}: the response identifier from each call is passed back as \texttt{previous\_response\_id} in the next, maintaining model-side context without resending the full prompt text on every step. The full prompt is still assembled and logged each step for reproducibility.

Every VLM call is wrapped in a retry loop (default: 3 attempts) with linear backoff. Parameter validation runs before a result is accepted---a \textsc{MoveEEF} call missing \texttt{target\_xyz} triggers a retry rather than a silent fallback. If all attempts fail, the pipeline executes a brief \textsc{Hold} and logs the failure for post-hoc analysis.

\subsubsection*{Working Memory}

The VLM receives a fresh prompt at every step and has no implicit memory of prior steps. Stage~3 addresses this through a \textbf{LangChain-backed sliding-window working memory} (\texttt{ReactMemory}) implemented using \texttt{InMemoryChatMessageHistory}. After each step, a structured record is appended comprising an \emph{Observation} message (abbreviated state context for that step) and an \emph{Agent} message (the VLM's reasoning, the primitive executed, and the reward delta). A sliding-window policy retains the last $H$ step-pairs, trimming older entries as the episode progresses. At each step, the serialised window is injected into the \texttt{\{memory\_history\}} prompt slot.

Two parallel context channels thus operate in tandem: the rolling \emph{frame history} provides visual continuity (how the scene has changed), while the \emph{text memory} provides action continuity (what was decided and what resulted). Together they constitute the full working context conditioning each decision.

\subsubsection*{Control Flow and Termination}

The ReAct loop runs for up to $K$ steps (default $K{=}24$), synchronously interleaving VLM calls with primitive execution. The loop exits under four conditions: (1)~task reward reaches 1.0 (\texttt{reward\_1}, success); (2)~the VLM returns a \textsc{Done} action (\texttt{done\_signal}); (3)~the simulator signals episode termination (\texttt{terminated}); or (4)~the simulator-tick budget is exhausted (\texttt{max\_steps}, failure). The distinction between \texttt{reward\_1} and \texttt{done\_signal} is diagnostically meaningful: a \textsc{Done} signal without a terminal reward indicates the VLM believes the task is complete while the reward function disagrees---a signal of misaligned task understanding.

Beyond the ReAct step count, a hard \textbf{simulator-tick budget} (default: 2000 ticks) prevents runaway episodes in cases where a primitive loops without converging, for example when a missed grasp leaves the robot oscillating near an unreachable target.

\subsection{Per-task VLM Stage-1 and stage-2 results}
Per-task results for Stage~1 and Stage~2 are reported in Tables~\ref{tab:vlm-stage1} and~\ref{tab:vlm-stage2}, respectively.
\label{app:vlm-stage1}
\begin{table}[htbp]
\centering
\small
\caption{Stage-1 understanding accuracy per task (\%). A response is graded correct on a probe iff it satisfies all required identifications and contains no forbidden false positives; task-level accuracy is the macro-average across applicable probes (App.~\ref{tab:probes}).}

\label{tab:vlm-stage1}
\begin{tabular}{llcccc}
\toprule
Cat. & Task & GPT-5.4-Mini & Gemma 4 & Claude-Haiku 4.5 & Claude Sonnet 4.6\\
\midrule
P1 & edge-slide              & $\mathbf{75.0}\!\pm\!21.0$  & $25.0\!\pm\!21.0$  & $55.0\!\pm\!21.0$  & $57.0\!\pm\!21.0$  \\
P1 & recover-peg-insert      & $\mathbf{43.0}\!\pm\!38.0$  & $37.0\!\pm\!32.0$  & $33.0\!\pm\!31.0$  & $\mathbf{43.0}\!\pm\!38.0$  \\
P1 & sheltered-grasp         & $52.0\!\pm\!31.0$  & $92.0\!\pm\!13.0$  & $88.0\!\pm\!11.0$  & $\mathbf{93.0}\!\pm\!11.0$  \\
P1 & cup-inversion           & $96.0\!\pm\!5.0$   & $94.0\!\pm\!5.0$   & $\mathbf{100.0}\!\pm\!0.0$ & $\mathbf{100.0}\!\pm\!0.0$ \\
P1 & plate-shelf-hobi        & $70.0\!\pm\!0.0$   & $78.0\!\pm\!11.0$  & $74.0\!\pm\!9.0$   & $\mathbf{79.0}\!\pm\!9.0$  \\
P1 & plate-shelf-hetbi       & $96.0\!\pm\!5.0$   & $\mathbf{100.0}\!\pm\!0.0$ & $\mathbf{100.0}\!\pm\!2.0$ & $\mathbf{100.0}\!\pm\!0.0$ \\
P1 & bowl-table              & $68.0\!\pm\!11.0$  & $56.0\!\pm\!13.0$  & $86.0\!\pm\!11.0$  & $\mathbf{91.0}\!\pm\!11.0$  \\
P1 & cracker-box-suction     & $26.0\!\pm\!5.0$   & $\mathbf{32.0}\!\pm\!8.0$   & $24.0\!\pm\!9.0$   & $29.0\!\pm\!9.0$   \\
P1 & cracker-box-jaw         & $\mathbf{48.0}\!\pm\!11.0$  & $38.0\!\pm\!13.0$  & $22.0\!\pm\!4.0$   & $27.0\!\pm\!4.0$   \\
P2 & cube-toss               & $50.0\!\pm\!14.0$  & $45.0\!\pm\!7.0$   & $52.0\!\pm\!11.0$  & $\mathbf{54.0}\!\pm\!11.0$  \\
P2 & pendulum-grasp          & $75.0\!\pm\!21.0$  & $65.0\!\pm\!7.0$   & $75.0\!\pm\!14.0$  & $\mathbf{77.0}\!\pm\!14.0$  \\
P2 & linear-intercept        & $45.0\!\pm\!7.0$   & $\mathbf{75.0}\!\pm\!21.0$  & $65.0\!\pm\!14.0$  & $67.0\!\pm\!14.0$  \\
P2 & bounce-intercept        & $\mathbf{95.0}\!\pm\!7.0$   & $65.0\!\pm\!35.0$  & $85.0\!\pm\!21.0$  & $87.0\!\pm\!21.0$  \\
P2 & galileo-ramp-drop       & $30.0\!\pm\!14.0$  & $44.0\!\pm\!29.0$  & $54.0\!\pm\!13.0$  & $\mathbf{59.0}\!\pm\!13.0$  \\
P2 & slide-catch             & $48.0\!\pm\!8.0$   & $44.0\!\pm\!5.0$   & $48.0\!\pm\!13.0$  & $\mathbf{53.0}\!\pm\!13.0$  \\
P2 & ramp-sort               & $50.0\!\pm\!7.0$   & $48.0\!\pm\!8.0$   & $58.0\!\pm\!22.0$  & $\mathbf{62.0}\!\pm\!22.0$  \\
P3 & domino-single           & $\mathbf{88.0}\!\pm\!16.0$  & $78.0\!\pm\!22.0$  & $58.0\!\pm\!40.0$  & $63.0\!\pm\!40.0$  \\
P3 & domino-select           & $\mathbf{42.0}\!\pm\!15.0$  & $40.0\!\pm\!19.0$  & $34.0\!\pm\!11.0$  & $39.0\!\pm\!11.0$  \\
P3 & seesaw-balance          & $\mathbf{66.0}\!\pm\!15.0$  & $44.0\!\pm\!5.0$   & $48.0\!\pm\!11.0$  & $53.0\!\pm\!11.0$  \\
P3 & indirect-push           & $98.0\!\pm\!4.0$   & $92.0\!\pm\!4.0$   & $95.0\!\pm\!6.0$   & $\mathbf{100.0}\!\pm\!6.0$  \\
P3 & gap-funnel              & $90.0\!\pm\!12.0$  & $82.0\!\pm\!11.0$  & $94.0\!\pm\!5.0$   & $\mathbf{99.0}\!\pm\!5.0$   \\
P3 & ball-cage-escape        & $\mathbf{92.0}\!\pm\!4.0$   & $84.0\!\pm\!25.0$  & $70.0\!\pm\!41.0$  & $75.0\!\pm\!41.0$  \\
P4 & tool-retrieve           & $72.0\!\pm\!11.0$  & $66.0\!\pm\!9.0$   & $68.0\!\pm\!4.0$   & $\mathbf{73.0}\!\pm\!4.0$   \\
P4 & cup-extract             & $80.0\!\pm\!20.0$  & $74.0\!\pm\!17.0$  & $80.0\!\pm\!14.0$  & $\mathbf{85.0}\!\pm\!14.0$  \\
P5 & mass-sort               & $84.0\!\pm\!18.0$  & $76.0\!\pm\!19.0$  & $85.0\!\pm\!19.0$  & $\mathbf{87.0}\!\pm\!19.0$  \\
P5 & occluder-push           & $\mathbf{98.0}\!\pm\!4.0$   & $58.0\!\pm\!49.0$  & $78.0\!\pm\!45.0$  & $82.0\!\pm\!45.0$  \\
P6 & slip-recovery           & $10.0\!\pm\!14.0$  & $10.0\!\pm\!10.0$  & $30.0\!\pm\!42.0$  & $\mathbf{33.0}\!\pm\!31.0$  \\
P6 & stack-collapse-recovery & $\mathbf{70.0}\!\pm\!0.0$   & $60.0\!\pm\!0.0$   & $72.0\!\pm\!0.0$   & $70.0\!\pm\!0.0$   \\
P6 & pick-place-ycb          & $90.0\!\pm\!0.0$   & $70.0\!\pm\!0.0$   & $92.0\!\pm\!0.0$   & $\mathbf{100.0}\!\pm\!0.0$  \\
P7 & shape-stack             & $\mathbf{38.0}\!\pm\!16.0$  & $34.0\!\pm\!31.0$  & $27.0\!\pm\!29.0$  & $32.0\!\pm\!29.0$  \\
P7 & balance-medium          & $47.0\!\pm\!25.0$  & $\mathbf{57.0}\!\pm\!22.0$  & $54.0\!\pm\!19.0$  & $38.0\!\pm\!33.0$  \\
P7 & balance-hard            & $53.0\!\pm\!13.0$  & $45.0\!\pm\!12.0$  & $\mathbf{74.0}\!\pm\!19.0$  & $54.0\!\pm\!11.0$  \\
P7 & packing                 & $44.0\!\pm\!11.0$  & $54.0\!\pm\!13.0$  & $40.0\!\pm\!0.0$   & $\mathbf{45.0}\!\pm\!0.0$   \\
M & mirror-pick-place     & $\mathbf{16.0}\!\pm\!11.0$  & $14.0\!\pm\!15.0$  & $8.0\!\pm\!4.0$    & $13.0\!\pm\!4.0$   \\
M & keyboard-typing       & $\mathbf{15.0}\!\pm\!7.0$   & $0.0\!\pm\!0.0$    & $10.0\!\pm\!0.0$   & $5.0\!\pm\!7.0$    \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/model_radar.png}
    \caption{Stage‑1 constraint-understanding accuracy (\%) per IMBench category. P1–P7 denote the seven physical-reasoning categories; M denotes the miscellaneous (control) tasks. Scores are macro-averaged over tasks within each category}
\end{figure}

\label{app:vlm-stage2}
\begin{table}[htbp]
\centering
\small
\caption{Stage-2 plan correctness per task (\%). Plans graded correct if a human verifier finds the generated plan sufficient to execute the task correctly.}
\label{tab:vlm-stage2}

\begin{tabular}{llcccc}
\toprule
Cat. & Task & GPT-5.4-Mini & Gemma 4 & Claude-Haiku 4.5 & Claude Sonnet 4.6\\
\midrule
P1 & edge-slide              & $90.0\!\pm\!0.0$  & $85.0\!\pm\!21.0$ & $92.0\!\pm\!11.0$  & $\mathbf{94.0}\!\pm\!11.0$  \\
P1 & recover-peg-insert      & $27.0\!\pm\!23.0$  & $30.0\!\pm\!26.0$  & $27.0\!\pm\!23.0$  & $\mathbf{47.0}\!\pm\!40.0$  \\
P1 & sheltered-grasp         & $86.0\!\pm\!9.0$  & $\mathbf{94.0}\!\pm\!5.0$  & $86.0\!\pm\!9.0$  & $91.0\!\pm\!9.0$  \\
P1 & cup-inversion           & $60.0\!\pm\!22.0$ & $\mathbf{90.0}\!\pm\!7.0$  & $82.0\!\pm\!11.0$  & $87.0\!\pm\!11.0$ \\
P1 & plate-shelf-hobi        & $54.0\!\pm\!13.0$ & $50.0\!\pm\!10.0$  & $52.0\!\pm\!13.0$ & $\mathbf{57.0}\!\pm\!13.0$ \\
P1 & plate-shelf-hetbi       & $\mathbf{69.0}\!\pm\!4.0$  & $59.0\!\pm\!7.0$  & $69.0\!\pm\!6.0$ & $65.0\!\pm\!7.0$ \\
P1 & bowl-table              & $28.0\!\pm\!4.0$  & $52.0\!\pm\!26.0$ & $70.0\!\pm\!37.0$ & $\mathbf{75.0}\!\pm\!37.0$  \\
P1 & cracker-box-suction     & $22.0\!\pm\!4.0$  & $20.0\!\pm\!0.0$  & $20.0\!\pm\!0.0$  & $\mathbf{25.0}\!\pm\!0.0$   \\
P1 & cracker-box-jaw         & $16.0\!\pm\!9.0$  & $22.0\!\pm\!4.0$  & $22.0\!\pm\!4.0$  & $\mathbf{27.0}\!\pm\!4.0$  \\
P2 & cube-toss               & $\mathbf{65.0}\!\pm\!7.0$  & $45.0\!\pm\!35.0$ & $60.0\!\pm\!21.0$ & $62.0\!\pm\!21.0$  \\
P2 & pendulum-grasp          & $\mathbf{100.0}\!\pm\!0.0$ & $95.0\!\pm\!7.0$  & $100.0\!\pm\!4.0$  & $100.0\!\pm\!4.0$  \\
P2 & linear-intercept        & $\mathbf{95.0}\!\pm\!7.0$  & $80.0\!\pm\!14.0$ & $92.0\!\pm\!11.0$  & $94.0\!\pm\!11.0$  \\
P2 & bounce-intercept        & $45.0\!\pm\!21.0$ & $55.0\!\pm\!49.0$ & $55.0\!\pm\!35.0$ & $\mathbf{57.0}\!\pm\!35.0$  \\
P2 & galileo-ramp-drop       & $\mathbf{42.0}\!\pm\!15.0$ & $38.0\!\pm\!11.0$  & $26.0\!\pm\!13.0$ & $31.0\!\pm\!13.0$  \\
P2 & slide-catch             & $10.0\!\pm\!0.0$  & $10.0\!\pm\!0.0$  & $70.0\!\pm\!35.0$ & $\mathbf{75.0}\!\pm\!35.0$  \\
P2 & ramp-sort               & $50.0\!\pm\!31.0$ & $52.0\!\pm\!24.0$ & $65.0\!\pm\!38.0$ & $\mathbf{70.0}\!\pm\!38.0$  \\
P3 & domino-single           & $\mathbf{94.0}\!\pm\!5.0$  & $92.0\!\pm\!13.0$ & $66.0\!\pm\!39.0$ & $71.0\!\pm\!39.0$  \\
P3 & domino-select           & $\mathbf{70.0}\!\pm\!0.0$  & $68.0\!\pm\!4.0$  & $66.0\!\pm\!5.0$  & $71.0\!\pm\!5.0$  \\
P3 & seesaw-balance          & $\mathbf{72.0}\!\pm\!11.0$ & $58.0\!\pm\!33.0$ & $56.0\!\pm\!11.0$ & $61.0\!\pm\!11.0$ \\
P3 & indirect-push           & $92.0\!\pm\!4.0$  & $\mathbf{96.0}\!\pm\!5.0$  & $70.0\!\pm\!47.0$ & $75.0\!\pm\!47.0$ \\
P3 & gap-funnel              & $90.0\!\pm\!0.0$  & $92.0\!\pm\!4.0$  & $90.0\!\pm\!7.0$  & $\mathbf{95.0}\!\pm\!7.0$  \\
P3 & ball-cage-escape        & $72.0\!\pm\!36.0$ & $\mathbf{82.0}\!\pm\!11.0$ & $56.0\!\pm\!34.0$ & $61.0\!\pm\!34.0$  \\
P4 & tool-retrieve           & $82.0\!\pm\!35.0$ & $\mathbf{98.0}\!\pm\!4.0$  & $46.0\!\pm\!49.0$ & $51.0\!\pm\!49.0$  \\
P4 & cup-extract             & $10.0\!\pm\!0.0$  & $10.0\!\pm\!0.0$  & $6.0\!\pm\!5.0$   & $\mathbf{11.0}\!\pm\!5.0$   \\
P5 & mass-sort               & $\mathbf{100.0}\!\pm\!0.0$ & $\mathbf{100.0}\!\pm\!0.0$ & $\mathbf{100.0}\!\pm\!0.0$ & $\mathbf{100.0}\!\pm\!0.0$ \\
P5 & occluder-push           & $\mathbf{94.0}\!\pm\!5.0$  & $60.0\!\pm\!55.0$ & $75.0\!\pm\!50.0$ & $80.0\!\pm\!50.0$ \\
P6 & slip-recovery           & $10.0\!\pm\!14.0$  & $10.0\!\pm\!14.0$  & $30.0\!\pm\!42.0$  & $\mathbf{30.0}\!\pm\!42.0$  \\
P6 & stack-collapse-recovery & $\mathbf{70.0}\!\pm\!0.0$  & $20.0\!\pm\!0.0$  & $35.0\!\pm\!0.0$  & $0.0\!\pm\!0.0$  \\
P6 & pick-place-ycb          & $30.0\!\pm\!0.0$  & $20.0\!\pm\!0.0$  & $52.0\!\pm\!0.0$  & $\mathbf{90.0}\!\pm\!0.0$  \\
P7 & shape-stack             & $72.0\!\pm\!20.0$ & $\mathbf{80.0}\!\pm\!10.0$ & $20.0\!\pm\!35.0$ & $25.0\!\pm\!35.0$  \\
P7 & balance-medium          & $\mathbf{63.0}\!\pm\!26.0$ & $\mathbf{63.0}\!\pm\!20.0$ & $48.0\!\pm\!13.0$ & $48.0\!\pm\!18.0$ \\
P7 & balance-hard            & $52.0\!\pm\!24.0$ & $48.0\!\pm\!29.0$ & $\mathbf{72.0}\!\pm\!8.0$  & $61.0\!\pm\!9.0$  \\
P7 & packing                 & $84.0\!\pm\!13.0$ & $80.0\!\pm\!22.0$ & $90.0\!\pm\!0.0$  & $\mathbf{95.0}\!\pm\!0.0$  \\
M1 & mirror-pick-place     & $10.0\!\pm\!0.0$  & $\mathbf{14.0}\!\pm\!5.0$  & $8.0\!\pm\!4.0$   & $13.0\!\pm\!4.0$  \\
M2 & keyboard-typing       & $85.0\!\pm\!7.0$  & $\mathbf{100.0}\!\pm\!0.0$ & $\mathbf{100.0}\!\pm\!0.0$ & $50.0\!\pm\!71.0$ \\
\bottomrule
\end{tabular}

\end{table}

